Keep Your Friends Close & Enemies Farther: Debiasing Contrastive Learning with Spatial Priors in 3D Radiology Images

Understanding of spatial attributes is central to effective 3D radiology image analysis where crop-based learning is the de facto standard. Given an image patch, its core spatial properties (e.g., position & orientation) provide helpful priors on expected object sizes, appearances, and structures through inherent anatomical consistencies. Spatial correspondences, in particular, can effectively gauge semantic similarities between inter-image regions, while their approximate extraction requires no annotations or overbearing computational costs. However, recent 3D contrastive learning approaches either neglect correspondences or fail to maximally capitalize on them. To this end, we propose an extensible 3D contrastive framework (Spade, for Spatial Debiasing) that leverages extracted correspondences to select more effective positive & negative samples for representation learning. Our method learns both globally invariant and locally equivariant representations with downstream segmentation in mind. We also propose separate selection strategies for global & local scopes that tailor to their respective representational requirements. Compared to recent state-of-the-art approaches, Spade shows notable improvements on three downstream segmentation tasks (CT Abdominal Organ, CT Heart, MR Heart).

==> section2_relatedworks.tex <==


\section{Related Works} \label{rel}

In this section, we focus on approaches directly relevant to volumetric medical image (VMI) representation learning and our adopted components. 
Thus, we omit self-supervised methods for videos, clustering-based approaches, and traditional metric learning.
For a more exhaustive review of contrastive methods, self-supervised learning (SSL), and image registration, we refer the readers to \cite{LKhc2020ContrastiveRL, liu2021selfsurvey,Duwairi2022SslMiaSurvey,hill2001medicalregistration,haskins2020deepregistration}. 


\subsection{Predictive \& Generative Self-supervision} \label{rel1}

Various \textbf{predictive pretext tasks} have been proposed to learn useful representations for volumetric medical images (VMIs). 
To effectively capture spatial information, previous works designed pretext tasks to predict
rotation \cite{zhu2020rubik}\cite{taleb20203dssl}, 
solve jigsaw puzzles \cite{zhuang2019selfrubik1}\cite{zhu2020rubik}\cite{taleb20203dssl}, 
recognize patch scales \cite{Zhang2021SARSR}, 
and infer relative locations of slices/patches/structures \cite{zhang2017selfslicepos}\cite{taleb20203dssl}\cite{nguyen2020selfpatchswaprelloc}\cite{bai2019selfXheart}.
Others predict transformations \cite{Qi2022LearningGTgeneraltransforms} or the presence of noise like corrupted slices \cite{nguyen2020selfpatchswaprelloc} \& masking \cite{zhu2020rubik}.

Alternatively, \textbf{generative approaches} learn representations by reconstructing original crops from noised inputs \cite{Chen2019SelfsupervisedLFcontextpred}.
Rubik++ \cite{tao2020revisiting} rotates crop segments and attempts to reconstruct the original alongside a discriminator for improved boundaries.
Models Genesis (MG) \cite{Zhou2019ModelsGG} proposes a set of effective noising strategies that outperforms cross-domain transfer learning \& spatial prediction tasks, and crucially highlights the importance of 3D pretraining for 3D tasks.
Complementing MG, TransVW \cite{zHaghighi2021TransferableVW} adds a classifier onto encoder features to discriminate anatomical concepts extracted from random crops of similar images.
Comparable to TransVW, our framework also uses MG except the reconstruction task takes a supplementary role since it contributes little to delivering a structured latent space and may neglect effective global representations. 
Also, the classification of anatomical concepts can be thought of as a discrete case of our approach where we similarly want corresponding regions to have similar representations.
Our method, however, does not require additional auto-encoder training \& disposal.


\subsection{Contrastive Self-supervision} \label{rel2}

\textbf{Contrastive learning methods in natural scene images} \cite{Wu2018UnsupervisedFLNonparam}\cite{Oord2018RepresentationLW}\cite{Chen2020ImprovedBW}\cite{chen2020simclr} adopt a metric learning approach by encouraging latent space representations of similar images to be close while features from distinct images are distanced.
Although highly effective in learning global representations of whole images, they neglect fine-grained local representations that are needed for dense prediction tasks.
DenseCL \cite{wang2021dense} addresses the local representation gap by adding a dense prediction head alongside a global projection head on encoder outputs.
This is not ideal for our applications since only the encoder is trained while recent works \cite{Zhou2021PreservationalLI}\cite{chaitanya2020contrastive} find pretrained decoders to improve downstream segmentation performance (we also affirm this observation; see \autoref{res2}).
VADeR \cite{o2020unsuperviseddense} amends this drawback by contrasting pixel representations from decoder outputs. 
However, VADeR utilizes an instance discrimination paradigm which is inappropriate for medical images with recurring structures, and only samples negative pixels from separate images which inhibits local understanding for intra-image regions.
Lastly, \cite{Wang2021ExploringCP} explores similar components like multi-scale memory banks and hard sampling, but does so in a fully supervised setting whereas our method requires no annotations.

\textbf{Effective negatives} are a key component in contrastive learning and false negatives worsen representations \cite{huynh2022boosting}.
Some reduce this biasing effect by reweighing the loss with positive samples in the denominator \cite{chuang2020debiasedcon}.
This works best under the assumption that there is a uniform number of positive classes, which is rarely the case in biomedical tasks.
Others focus on hard negative sampling \cite{kalantidis2020hard}\cite{Wang2021ExploringCP} which offer more gradient contributions, or combine the two principles \cite{Robinson2021ContrastiveLWithHardNeg}.
We make different assumptions about class distributions and use spatial priors as a positive correlator to semantic similarity.
Furthermore, we find that debiasing by assigning appropriate positives \& negatives learns effective representations. We leave additional techniques like hard sampling to future exploration.

\textbf{Contrastive works in 3D medical images} directly adapt various natural scene approaches like CPC \cite{taleb20203dssl} and MoCo \cite{chen2021momentumcovidclassif} for representation learning. 
Others combine contrastive approaches with auxiliary tasks such as reconstruction \cite{Taher2022CAiDCI}.
PCRL \cite{Zhou2021PreservationalLI} additionally proposes model mixup and a transformation-based attention module to regularize representations.
However, these approaches only learn global contrastive features, and neglect spatial priors \& sample diversity by only selecting same-image positives. 
For more diverse positive samples, the methods in\cite{vu2021medaug}\cite{Sowrirajan2021MoCoPIMetadata}\cite{azizi2021bigmedical} leverage patient identities or metadata in 2D images. 
In the context of 3D radiology, GLCL \cite{chaitanya2020contrastive} \& PCL \cite{Zeng2021PositionalCL} leverage spatial priors by assuming slices in corresponding volumes contain similar anatomical structures. 
These approaches work on 2D slices, which is disadvantageous as discussed in \textbf{(1)} (see \autoref{intro}).
There exists alternative methods (e.g., PGL \cite{Xie2020PGLPL}) that entirely omit negative samples and utilize only positives with gradient stopping to prevent representational collapse. 
However, negative samples are important to metric learning \cite{Kaya2019DeepMetricLearningSurvey}, especially in medical images given their homogeneous appearances across images. 
We show that negatives generally improve downstream performance (see Table \ref{tab:main} \& \autoref{res2}).

Other works adopt local contrastive techniques with voxel embeddings for point matching \cite{yan2022sam}, superpixels for few-shot segmentation \cite{ouyang2020selfcontrsuperpixelfewshot}, or multiple contrastive objects for semi-supervised segmentation \cite{you2022simcvd}.
These either aren't designed for segmentation, are sensitive to the quality of extracted superpixels, or require dense annotations, respectively.

% SAM \cite{yan2022sam} trains both global and local embeddings for learning point correspondences. 
% Segmentation requires more than point-wise discriminative features but local and global context as well. 
% For few shot image segmentation, \cite{ouyang2020selfcontrsuperpixelfewshot} contrasts superpixel embeddings.
% \cite{you2022simcvd} makes use of both labeled \& unlabeled images and use contrastive losses to augment segmentation performance. 
% These methods propose relatively complex superpixel extraction or multi-task training with dense annotations. 

\subsection{Medical Image Registration} \label{rel3}

Automatic registration of medical images is a widely studied topic where the objective is to learn a spatial mapping $T$ from one image or coordinate space $\Omega_A$ to another image or coordinate space $\Omega_B$ so that image contents are aligned. 
% This is useful for longitudinal studies to track disease progression, or population studies to understand anatomical variations.
Approaches are either linear (e.g., rigid \& affine) or deformable.
% where local correspondences are more accurately computed.
% images are first globally aligned through affine transformations and local correspondences are then iteratively computed. 

Traditional techniques \cite{hill2001medicalregistration} often iteratively optimize an energy function via a similarity metric (e.g., normalized cross-correlation).
In contrast, recent learning-based works propose supervised \cite{yang2017quicksilver} and unsupervised approaches \cite{balakrishnan2019voxelmorph,kim2021cyclemorph}.

For our task, we are interested in finding global correspondences between image regions such that there is approximate anatomical concurrence. 
We show that rough alignment through affine registration is fast, effective, and sufficient. 

% including mean squared error~\cite{beg2005computing}, sum of squared differences~\cite{wolberg2000robust}, normalized cross-correlation~\cite{avants2008symmetric}, and mutual information~\cite{viola1997alignment}. \comments{TMIs???}
%
% However, these algorithms are highly time consuming due to the high dimensionality of the parameter space, especially when dealing with deformable registration. 
%

% Recently, learning-based approaches have been proposed. There are two main types of methods. (1) Supervised methods, which require a ground truth deformable field that either produced by synthetically or generated by traditional registration methods for training~\cite{yang2017quicksilver,sokooti2017nonrigid,cao2018deep}. (2) Unsupervised methods, which learn the registration representation (i.e., deformable field) by aligning image pair via spatial transfomrer network, without utilizing the ground truth deformable field~\cite{de2019deep,balakrishnan2019voxelmorph,dalca2019unsupervised,kim2021cyclemorph}.
%




